The McDonald Accelerating Stars Survey (MASS): Discovery of a Long-Period Substellar Companion Orbiting the Old Solar Analog HD 47127

Brown dwarfs with well-determined ages, luminosities, and masses provide rare but valuable tests of low-temperature atmospheric and evolutionary models. We present the discovery and dynamical mass measurement of a substellar companion to HD 47127, an old ($\approx$7-10 Gyr) G5 main sequence star with a mass similar to the Sun. Radial velocities of the host star with the Harlan J. Smith Telescope uncovered a low-amplitude acceleration of 1.93 $\pm$ 0.08 m s$^{-1}$ yr$^{-1}$ based on 20 years of monitoring. We subsequently recovered a faint ($\Delta H$=13.14 $\pm$ 0.15 mag) co-moving companion at 1.95$''$ (52 AU) with follow-up Keck/NIRC2 adaptive optics imaging. The radial acceleration of HD 47127 together with its tangential acceleration from Hipparcos and Gaia EDR3 astrometry provide a direct measurement of the three-dimensional acceleration vector of the host star, enabling a dynamical mass constraint for HD 47127 B (67.5-177 $M_\mathrm{Jup}$ at 95% confidence) despite the small fractional orbital coverage of the observations. The absolute $H$-band magnitude of HD 47127 B is fainter than the benchmark T dwarfs HD 19467 B and Gl 229 B but brighter than Gl 758 B and HD 4113 C, suggesting a late-T spectral type. Altogether the mass limits for HD 47127 B from its dynamical mass and the substellar boundary imply a range of 67-78 $M_\mathrm{Jup}$ assuming it is single, although a preference for high masses of $\approx$100 $M_\mathrm{Jup}$ from dynamical constraints hints at the possibility that HD 47127 B could itself be a binary pair of brown dwarfs or that another massive companion resides closer in. Regardless, HD 47127 B will be an excellent target for more refined orbital and atmospheric characterization in the future.

==> hd47127_rvs_tull.tex <==
\begin{deluxetable}{lcc}
\renewcommand\arraystretch{0.9}
\tabletypesize{\small}
\setlength{ \tabcolsep } {.1cm}
\tablewidth{0pt}
\tablecolumns{3}
\tablecaption{Tull Spectrograph Relative Radial Velocities of HD47127\label{tab:hd47127_rvs}}
\tablehead{
    \colhead{Date}  & \colhead{RV} & \colhead{$\sigma_{\mathrm{RV}}$} \\
    \colhead{(BJD)} & \colhead{(m s$^{-1}$)} & \colhead{(m s$^{-1}$)}
        }
\startdata
%========================================================
%           Date    &          RV    &      RV_err   \\
%========================================================
   2452037.59844    &        20.7    &         5.0   \\
   2452221.93066    &        13.9    &         3.8   \\
   2452248.87150    &        16.1    &         5.6   \\
   2452249.85430    &         7.8    &         5.2   \\
   2452306.76529    &         6.5    &         4.7   \\
   2452326.70915    &        34.9    &         4.3   \\
   2452330.68521    &        26.8    &         4.3   \\
   2452331.66394    &        23.3    &         4.2   \\
   2452357.65539    &        31.2    &         4.5   \\
   2452577.97230    &         4.8    &         4.0   \\
   2452597.99066    &        17.6    &         4.4   \\
   2452598.95448    &        16.3    &         4.1   \\
   2452620.97803    &        19.1    &         4.4   \\
   2452659.85618    &        33.2    &         4.8   \\
   2452743.67414    &         3.4    &         4.8   \\
   2452932.98742    &         5.2    &         5.2   \\
   2452959.94374    &         9.9    &         4.4   \\
   2453017.87908    &        26.6    &         4.8   \\
   2453037.82070    &        30.4    &         5.6   \\
   2453075.70032    &        16.0    &         4.4   \\
   2453321.94197    &        17.9    &         7.4   \\
   2453636.95392    &         8.7    &         4.7   \\
   2453689.90429    &        23.9    &         4.5   \\
   2453747.76228    &        13.0    &         8.5   \\
   2453787.73893    &        30.2    &         4.5   \\
   2453808.73991    &        11.8    &         4.6   \\
   2454017.98926    &        -1.1    &         4.6   \\
   2454114.78849    &        21.4    &         5.4   \\
   2454557.66250    &         3.3    &         6.8   \\
   2454816.91344    &        -0.7    &         5.8   \\
   2454838.65782    &        -3.6    &         6.3   \\
   2455136.97894    &         5.0    &         7.4   \\
   2455285.63541    &        12.3    &         5.0   \\
   2455499.98600    &         1.6    &         4.5   \\
   2455528.87689    &         5.2    &         4.6   \\
   2455549.79868    &        -7.7    &         4.4   \\
   2455587.80622    &        -2.4    &        10.9   \\
   2455588.77472    &        18.3    &         5.5   \\
   2455616.73483    &         9.9    &         4.6   \\
   2455634.69704    &        -0.2    &         4.4   \\
   2455643.65943    &        -3.1    &         4.7   \\
   2455842.91355    &        -9.4    &         5.4   \\
   2455873.93798    &         2.7    &         6.2   \\
   2455990.70303    &       -10.4    &         5.3   \\
   2456236.94204    &         7.3    &         4.2   \\
   2456267.77929    &        -2.7    &         4.2   \\
   2456315.74827    &        -2.4    &         4.7   \\
   2456352.71810    &        -1.0    &         5.1   \\
   2456372.68742    &        -2.0    &         4.3   \\
   2456402.61755    &        -1.4    &         4.6   \\
   2456560.97240    &       -20.2    &         4.5   \\
   2456588.98514    &        -4.2    &         4.5   \\
   2456589.90170    &        -1.2    &         4.6   \\
   2456590.90299    &        13.4    &         8.9   \\
   2456592.01130    &        -5.1    &         4.6   \\
   2456592.93472    &         4.6    &         5.1   \\
   2456593.80418    &        -8.3    &         4.7   \\
   2456593.99562    &       -12.2    &         4.0   \\
   2456612.87715    &       -16.6    &         4.3   \\
   2456612.90371    &       -14.7    &         4.5   \\
   2456613.85796    &        -6.7    &         4.2   \\
   2456623.83550    &        -1.6    &         4.2   \\
   2456623.98465    &        -1.8    &         5.4   \\
   2456624.81372    &        -4.7    &         4.7   \\
   2456624.97991    &        -1.1    &         4.6   \\
   2456625.80718    &         0.4    &         4.6   \\
   2456640.83738    &       -10.6    &         4.8   \\
   2456640.94564    &        -4.5    &         5.0   \\
   2456641.78970    &       -13.4    &         4.6   \\
   2456641.94238    &        -8.9    &         4.4   \\
   2456642.76415    &        -8.2    &         4.6   \\
   2456642.96746    &        -5.1    &         4.3   \\
   2456643.91416    &        -6.5    &         4.6   \\
   2456671.82293    &         0.8    &         4.3   \\
   2456675.77383    &        -6.4    &         4.6   \\
   2456696.70459    &        17.6    &         9.7   \\
   2456727.66926    &        -5.4    &         4.9   \\
   2456756.62371    &        -6.2    &         6.3   \\
   2456936.97725    &        -6.5    &         4.8   \\
   2456969.90959    &        -3.7    &         4.2   \\
   2457004.87040    &       -12.2    &         4.8   \\
   2457033.81768    &        -6.6    &         4.8   \\
   2457059.71078    &        -3.2    &         4.5   \\
   2457092.69039    &        -1.2    &         4.6   \\
   2457109.68419    &       -17.9    &         5.1   \\
   2457119.60622    &        -6.1    &         5.0   \\
   2457156.62160    &         0.6    &         8.3   \\
   2457281.97958    &       -15.0    &         5.1   \\
   2457340.02868    &        -4.2    &         4.3   \\
   2457672.98697    &         5.5    &         5.8   \\
   2457735.92176    &       -14.2    &         4.5   \\
   2457739.89325    &       -15.8    &         4.0   \\
   2457770.82315    &        -7.5    &         4.6   \\
   2457796.71582    &        -8.7    &         4.9   \\
   2457834.66440    &        -3.2    &         4.8   \\
   2457847.64098    &        -3.7    &         4.9   \\
   2457850.66161    &        -6.8    &         4.6   \\
   2458042.98327    &       -16.9    &         4.7   \\
   2458067.83344    &        -1.8    &         4.5   \\
   2458096.93581    &        -9.5    &         4.6   \\
   2458144.78789    &        -8.4    &         4.6   \\
   2458172.77562    &         0.9    &         4.9   \\
   2458184.71916    &        -2.4    &         4.5   \\
   2458215.64864    &        -1.7    &         5.2   \\
   2458457.84961    &        -1.3    &         9.2   \\
   2458465.86606    &       -25.5    &         5.3   \\
   2458515.84603    &         0.3    &         5.3   \\
   2458529.69560    &        -5.3    &         5.1   \\
   2458779.95684    &       -21.1    &         4.4   \\
   2458806.94336    &       -20.7    &         5.3   \\
   2458856.88066    &       -19.1    &         5.0   \\
   2458958.63388    &        -9.9    &         4.8   \\
   2459146.00450    &       -25.4    &         4.6   \\
   2459171.00689    &       -24.2    &         5.2   \\
   2459191.91037    &         3.7    &         5.6   \\
   2459203.77569    &       -18.0    &         5.0   \\
   2459227.83318    &       -14.7    &         5.1   \\
   2459240.77065    &       -19.6    &         4.6   \\
\enddata
\end{deluxetable}

